NAS-Bench-1Shot1: Benchmarking and Dissecting One-shot Neural Architecture Search

One-shot neural architecture search (NAS) has played a crucial role in making NAS methods computationally feasible in practice. Nevertheless, there is still a lack of understanding on how these weight-sharing algorithms exactly work due to the many factors controlling the dynamics of the process. In order to allow a scientific study of these components, we introduce a general framework for one-shot NAS that can be instantiated to many recently-introduced variants and introduce a general benchmarking framework that draws on the recent large-scale tabular benchmark NAS-Bench-101 for cheap anytime evaluations of one-shot NAS methods. To showcase the framework, we compare several state-of-the-art one-shot NAS methods, examine how sensitive they are to their hyperparameters and how they can be improved by tuning their hyperparameters, and compare their performance to that of blackbox optimizers for NAS-Bench-101.

==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/0_abstract.tex <==
\begin{abstract}
One-shot neural architecture search (NAS) has played a crucial role in making NAS methods computationally feasible in practice.
%the advancement and democratization of research in NAS as a subfield of AutoML. 
Nevertheless, there is still a lack of understanding on how these weight-sharing algorithms exactly work due to the many factors controlling the dynamics of the process.
%, and as a result, a large number of variants have been proposed in different research papers. 
%
%In order to allow a proper empirical evaluation without confounding factors that yields 
In order to allow a scientific study of these components, 
%without the confounding factors introduced by different code bases, 
we introduce a general framework for one-shot NAS that can be instantiated to many recently-introduced variants and introduce a general benchmarking framework that draws on the recent large-scale tabular benchmark NAS-Bench-101 for cheap anytime evaluations of one-shot NAS methods. 
%by mapping their anytime solutions to their representation in NAS-Bench-101. 
%
To showcase the framework, we compare several state-of-the-art one-shot NAS methods, examine how sensitive they are to their hyperparameters and how they can be improved by tuning their hyperparameters, and compare their performance to that of blackbox optimizers for NAS-Bench-101.
%Finally, we examine how the hyperparameters of a one-shot NAS method affect the search by wrapping it with a black box optimizer. We compare these results with discrete NAS optimizers and demonstrate that gradient-based NAS methods outperform them, particularly on our largest search space.
%\notejs{Added things to the end.}
\end{abstract}

==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/1_introduction.tex <==
\section{Introduction}
\label{sec: introduction}

%Neural architecture search (NAS) has attracted a lot of attention in recent years due its conceptual simplicity and effectiveness in finding network architectures which outperform human-designed ones both in terms of model performance and size~\citep{zoph-iclr17, zoph-arXiv18, real17a, real-arXiv18a}.
While neural architecture search (NAS) has attracted a lot of attention due to the effectiveness in automatically designing state-of-the-art neural networks~\citep{zoph-iclr17, zoph-arXiv18, real17a, real-arXiv18a}, the focus has recently shifted to making the search process more efficient~\citep{Pham18,Elsken19,darts,Xie18,Cai19,casale2019}. 
The most crucial concept which led to a reduction in search costs to the order of a single function evaluation is certainly the weight-sharing paradigm: Training only a single large architecture (the \textit{one-shot} model) subsuming all the possible architectures in the search space~\citep{brock2018smash,Pham18}.
%This has led to a reduction in search costs to the order of a single function evaluation~\citep{brock2018smash,enas,Elsken19,darts,Xie18,Cai19,casale2019}. 

Despite the great advancements of these methods, the exact results of many NAS papers are often hard to reproduce~\citep{li2019random,sciuto19,Yang2020NAS}. This is a result of several factors, such as unavailable original implementations, differences in the employed search spaces, training or evaluation pipelines, hyperparameter settings, and even pseudorandom number seeds~\citep{best_practices}.
%, complicate a direct comparison of NAS optimizers. 
%
%, such as the hardware or deep learning libraries used
%(see~\citet{}).
One solution to guard against these problems would be a common library of NAS methods that provides primitives to construct different algorithm variants, similar to what as RLlib~\citep{rllib} offers for the field of reinforcement learning. Our paper makes a first step into this direction.

Furthermore, experiments in NAS can be computationally extremely costly, making it virtually impossible to perform proper scientific evaluations with many repeated runs to draw statistically robust conclusions.
To address this issue, \citet{ying19a} introduced NAS-Bench-101, a large tabular benchmark with 423k unique %ResNet-like~\citep{he-cvpr16} and Inception-like~\citep{szegedy-15, szegedy-16a, szegedy-16b} 
cell architectures, trained and fully evaluated using a one-time extreme amount of compute power (several months on thousands of TPUs), which now allows to cheaply simulate an arbitrary number of runs of NAS methods, even on a laptop. NAS-Bench-101 enabled a comprehensive benchmarking of many discrete NAS optimizers~\citep{zoph-iclr17, real-arXiv18a}, using the exact same settings. However, the discrete nature of this benchmark does not allow to directly benchmark one-shot NAS optimizers~\citep{Pham18, darts, Xie18, Cai19}.
In this paper, we introduce the first method for making this possible.
%reusing the NAS-Bench-101 space to benchmark one-shot NAS methods.

Specifically, after providing some background (Section \ref{sec:background}), we make the following contributions:

%(rather than the validation error of the one-shot (search) model.
%
%NAS-Bench-1Shot1 includes 3 subspaces of the original NAS-Bench-101 space, which we utilize these subspaces to evaluate the one-shot NAS optimizers and report their anytime performance, which is the validation or test error of individual (discrete) architectures queried from the NAS-Bench-101 table and not the validation error of the one-shot (search) model. 
%Previous work \citep{bender_icml:2018,sciuto19} analyzed the impact that the weight sharing mechanism has on the optimization process, but no prior analysis had access to a sufficiently large fully evaluated search space. 
%Therefore, open questions remain regarding how correlated the surrogate objective of the NAS optimizer is to the resulting architectures' test performance. An additional interesting question is how the hyperparameters of the one-shot model and optimizer affect the search.

%To provide a thorough answer to these questions, we use NAS-Bench-101~\citep{ying19a}, which provides us with an exhaustive evaluation of 423k unique convolutional architectures on CIFAR-10. 
%Our proposed analysis maps the graph representation of several one-shot NAS optimizers~\citep{darts,li2019random,dong2019search} to subspaces of the NAS-Bench-101 search space. This enables us to follow the full trajectory of architectures found by each method at each search epoch without the need for retraining them from scratch, allowing for a careful analysis.

%To answer these questions, after describing background (Section \ref{sec:background}), we make the following contributions:
\begin{enumerate}[leftmargin=*]
    \item  We introduce \emph{NAS-Bench-1Shot1}, 
    a novel benchmarking framework that allows us to reuse the extreme amount of compute time that went into generating NAS-Bench-101~\citep{ying19a} to cheaply benchmark one-shot NAS methods. Our mapping between search space representations is novel to the best of our knowledge and it allows querying the performance of found architectures from one-shot NAS methods, contrary to what is claimed by \citet{ying19a}.
    Specifically, it allows us to follow the full trajectory of architectures found by arbitrary one-shot NAS methods at each search epoch without the need for retraining them individually, allowing for a careful and statistically sound analysis (Section\mbox{ \ref{sec:methodology}}).
%    for benchmarking the anytime performance of one-shot NAS methods as the validation (or test) error of individual (discrete) architectures queried from the NAS-Bench-101 table.
% This reinterpretation of the NASBench search space enables us to follow the full trajectory of architectures found by all methods at each search epoch without the need for retraining them individually, allowing for a careful and statistically sound analysis (Section \ref{sec:methodology}).
%    \item We use this analysis to benchmark 4 different state-of-the-art one-shot NAS optimizers. The optimizers were built upon the same code base to eliminate confounding factors, which would make a comparison less meaningful.
    %Our methodology allows to circumvent the architecture evaluation phase of many NAS optimizers, in which a found architecture is trained from scratch in a higher parameterized model, as we can query the results from NAS-Bench-101.
    \item We introduce a general framework for one-shot NAS methods that can be instantiated to many recent one-shot NAS variants, enabling fair head-to-head evaluations based on a single code base (Section \ref{sec:framework}).
    \item We use the above to compare several state-of-the-art one-shot NAS methods,
    assess the correlation between their one-shot model performance and final test performance,
    examine how sensitive they are to their hyperparameters,
    %and how they can be improved by careful regularization,
    and compare their performance to that of black-box optimizers used in NAS-Bench-101 (Section \ref{sec:experiments}).
%    \item We show that there is almost no correlation between the test errors of the individual architectures retrained from scratch and when evaluated using the one-shot model parameters.
%    As we observe a non-robust behavior of the one-shot NAS optimizers, we wrap the NAS search procedure with a black box optimizer and tune the hyperparameters affecting this robustness tailored to minimize the true objective (validation error of the fully evaluated discrete architectures), rather than the one-shot validation error.
% \notejs{Maybe we can say that this allows for a comparable analysis to existing discrete optimizers such as Regularized Evolution.}
\end{enumerate}

We provide our open-source implementation\footnote{\href{https://github.com/automl/nasbench-1shot1}{https://github.com/automl/nasbench-1shot1}}, which we expect will also facilitate the reproducibility and benchmarking of other one-shot NAS methods in the future.
%\notefh{Where do you provide this code? It'd be good to use an anonymous github repo (created using a new anonymous gmail address), where you include code without reference to any of our identities.}
%\noteaz{Yes, we will add an anonymous repo as a link here.}

==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/2_background.tex <==
\section{Background and Related Work}
\label{sec:background}

\subsection{NAS-Bench-101}\label{sec: NAS-Bench}
NAS-Bench-101 \citep{ying19a} is a database of an exhaustive evaluation of all architectures in a constrained cell-structured space on CIFAR-10 \citep{krizhevsky-tech09a}. Each cell is represented as a directed acyclic graph (DAG) where the nodes represent operation choices and the edges represent the information flow through the neural network (see also Figure \ref{fig:sec2:overview_graphic} and Section \ref{subsec: search_spaces}). To limit the number of architectures in the search space, the authors used the following constraints on the cell: 3 operations in the operation set $\mathcal{O}$ = \{3x3 convolution, 1x1 convolution,  3x3 max-pool\}, at most 7 nodes (this includes input and output node, therefore 5 choice nodes) and at most 9 edges.

These constraints, and exploiting symmetries, reduced the search space to 423k unique valid architectures. Each architecture was trained from scratch three times to also obtain a measure of variance. In addition, each architecture was trained for 4, 12, 36 and 108 epochs; for our analysis, we mainly used the results for models trained for 108 epochs, if not stated otherwise.

%In their work, \citet{ying19a} compared different discrete optimizers on NASBench.

\subsection{NAS-Bench-102}\label{sec: NAS-Bench-102}
Concurrently to this work, ~\citet{dong20} released NAS-Bench-102, which is another NAS benchmark that, differently from NAS-Bench-101, enables the evaluation of weight-sharing NAS methods. Their search space consists of a total of 15,625 architectures, which is exhaustively evaluated on 3 image classification datasets. Similarly to \citet{zela19} and this work, \citet{dong20} found that architectural overfitting occurs for DARTS for all their datasets.

While NAS-Bench-102 and this work go towards the same direction, they differ in many ways:
\begin{enumerate}[leftmargin=*]
    \item They use extensive computation to create a \emph{new} benchmark (with 15.625 architectures), while we devise a novel reformulation to reuse the even much more extensive computation of the NAS-Bench-101 dataset (~120 TPU years) to create three new one-shot search spaces with the larges one containing 363.648 architectures. This required zero additional computational cost.
    \item We show that it \emph{is} possible to reuse the graph representation in NAS-Bench-101 to run one-shot NAS methods; this requires changes to the one-shot search space, but allows a mapping which can be used for architecture evaluation.
    \item They evaluate their search space on 3 image classification datasets, while we introduce 3 different search spaces (as sub-spaces of NAS-Bench-101) with growing complexity.
\end{enumerate}

\subsection{One-shot Neural Architecture Search}\label{subsec: oneshotNAS}
The NAS problem can be defined as searching for the optimal operation (e.g. in terms of validation error of architectures) out of the operation set $\mathcal{O}$ in each node of the DAG and for the best connectivity pattern between these nodes.
%Of course, this combinatorial optimization problem is subject to certain constraints, e.g. at most 9 edges for the NAS-Bench-101 search space.

Designing architectures for optimized accuracy or to comply with resource constraints led to significant breakthroughs on many standard benchmarks \citep{Pham18, zoph-iclr17, brock2018smash, darts, Cai19, Elsken19}. 
%
While early methods were computationally extremely expensive \citep{zoph-iclr17}, the weight-sharing paradigm~\citep{brock2018smash,Pham18} led to a significant increase in search efficiency. Here, the weights of the operations in each architecture are shared in a supermodel (the so-called \emph{one-shot model} or convolutional neural fabric~\citep{SaxenaV16}), 
%@Arber: please check
which contains an exponential number of sub-networks, each of which represents a discrete architecture. Architectures whose sub-networks share components (nodes/edges)
%in the DAG representation 
also share the weights for these components' operations; therefore, in analogy to DropOut~\citep{srivastava-jmlr14a}, training one architecture implicitly also trains (parts of) an exponential number of related architectures.
%
%allowing these architectures to reuse already well-trained operations from other architectures.
%For example, if two sampled architectures in the one-shot model would have a common node in the DAG representation, also the parameters of the operations in these nodes would be shared. 
There are a variety of methods on how to conduct NAS by means of the one-shot model~\citep{brock2018smash, Pham18, bender_icml:2018, darts, li2019random} (see also Appendix \ref{sec:app:optimizers}), but the final problem is to find the optimal sub-network in this one-shot model.

The weight sharing method was used to great effect in DARTS~\citep{darts}, where it allows a gradient based optimization of both the architectural and the one-shot weights. Subsequent work on DARTS has addressed further lowering the computational and the memory requirements \citep{dong2019search, xu2019pcdarts, Cai19, casale2019}.

One fundamental drawback of the weight sharing method is the fact that the architecture search typically takes place in a lower fidelity model (e.g., using less cells and/or cheaper operations): the so-called \emph{proxy model}. After the search, a discrete architecture is derived from the proxy model which is then trained with more parameters --- a stage often referred to as \emph{architecture evaluation}. This poses the question whether the architecture found in the proxy model is also a good architecture in the bigger model,
a question studied by several recent works \citep{bender_icml:2018, sciuto19}.

% Mention something about the analysis bender, sciuto

==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/3_methods.tex <==
\section{A general framework for benchmarking one-shot NAS}
\label{sec:methodology}
%\notefh{Structure: the only subsection of this section is the search space representation. Is that what the general benchmarking framework amounts to, or is there more to this (such as an open-source implementation of the different algorithms), using the same code base to remove any confounding factors? As argued in the best practices arXiv note, this is really important, and we should clearly claim this as a contribution of this paper (also explicitly in the bullet point list of contributions above).}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\textwidth]{imgs/search_space/search_space_visualization.pdf}
\caption{Overview of the NAS-Bench-1Shot1 analysis strategy. 
%@Arber: please check
The one-shot model we construct only contains discrete architectures that are elements of NAS-Bench-101~\citep{ying19a}.
%A one-shot model is constructed which only contains discrete architectures which are a subspace of NAS-Bench-101~\citep{ying19a}. 
The cell architecture chosen is similar to that of \citet{bender_icml:2018}, with each choice block containing an operation decision. Note that NAS-Bench-101 does not contain a separate reduction cell type. Plot on the right from~\citet{ying19a} (Best viewed in color).
}
\label{fig:sec2:overview_graphic}
\end{figure}

We will now introduce our framework for cheaply benchmarking the anytime performance of one-shot NAS methods.
Our main analysis strategy is the following: First, we run the search procedure of various methods and save the architecture weights of the one-shot models for each epoch. Second, we find the discrete architecture at each epoch and query it in NAS-Bench-101. The last step is not trivial due to the different representations of the search space used in NAS-Bench-101 and standard one-shot methods. \citet{ying19a} state that one-shot methods cannot be directly evaluated on NAS-Bench-101. In the following sections we present a mapping between these different search space representations, which eventually enable us to evaluate one-shot methods on NAS-Bench-101. To the best of our knowledge this is a novel contribution of this paper.
%This analysis requires that we designed our one-shot search space to only contain discrete architectures which are also contained in NASBench .
%\notefh{Probably drop this intermediate preview; we want only one such preview in the beginning, as part of the bullet-point list of contributions.}
%We describe in Section \ref{subsec: search_spaces} the search space design. Section \ref{subsec: evaluation_procedure} explains how we find the corresponding discrete architecture to query in NASBench for a given set of architectural weights. Finally, Section \ref{subsec: optimization_pipeline} provides further details on the implementation of the one-shot NAS optimizers.

\subsection{Search space representation}
\label{subsec: search_spaces}

In order to carry out the analysis we propose in this work, we had to construct a search space that only contains discrete architectures that are also contained in NAS-Bench-101. This allows us to look up any discrete architectures' performance in NAS-Bench-101 when the larger model is trained from scratch. Unfortunately, this is non-trivial since the NAS-Bench-101 space does not match the typical space used in one-shot NAS methods. We separately consider the various parts of the search space.
%network-level and the cell-level topology. 
%\noteazout{Restructured and rewrote most of the text}

\textbf{Network-Level Topology.} In terms of network-level topology, our search spaces closely resemble the models which were evaluated in NAS-Bench-101. We used the same macro architecture as in NAS-Bench-101, i.e., 3 stacked blocks with a max-pooling operation in-between, where each block consists of 3 stacked cells (see Figure~\ref{fig:sec2:overview_graphic}).
While our final evaluation models exactly follow NAS-Bench-101 in order to be able to reuse its evaluations, our one-shot model only has 16 initial convolution filters, rather than the 128 used in NAS-Bench-101. This is a common practice to accelerate NAS and used similarly in, e.g., \citet{darts}. 

\textbf{Cell-Level Topology.} The cell-level structure is represented as a DAG, where the input node is the output of a previous cell or the convolutional stem (projected using a $1\times 1$ convolution in order to scale the channel counts), and the output node consists of firstly concatenating the outputs of all intermediate nodes and adding to that the projected output of the input node. In order to have the operation choices still in the intermediate nodes of the DAG, we adapt the \textit{choice block} motif from \citet{bender_icml:2018} as depicted in Figure~\ref{fig:sec2:overview_graphic}. The edges connecting input, output nodes and choice blocks represent only the information flow in the graph. To have a large and expressive enough search space(s), we introduce the following architectural weights in the DAG edges:
\begin{itemize}[leftmargin=*]
    \item $\alpha^{i,j}$ to edges connecting nodes $i<j$ to choice block $j$. The input of choice block $j$ is then computed as $I^j = \sum_{i<j} \frac{\exp(\alpha^{i,j})}{\sum_{i^{\prime} < j}\exp(\alpha^{i^{\prime},j})} x^i$, where $x^i$ is the output tensor of node $i$ (either input node or choice block).
    \item $\gamma^{j,k}$ to the edges connecting the input node or choice blocks $j<k$ to the output node $k$ of the cell, where the corresponding output feature maps of the choice blocks are concatenated and then added to the projected input of the cell: $O^k = \frac{\exp(\gamma^{1,k})}{\sum_{j^{\prime} < k}\exp(\gamma^{j^{\prime},k})} x^1 + \oplus_{1<j<k} \frac{\exp(\gamma^{j,k})}{\sum_{j^{\prime} < k}\exp(\gamma^{j^{\prime},k})} x^j$, where $\oplus$ is the concatenation operator and $x^1$ the input node tensor.
\end{itemize}

%The common search space by \citet{zoph-arXiv18} which is also used by DARTS \citep{darts} has a key drawback which made it infeasible to use in this analysis. Any cell contained in NASBench is constrained to have at most 9 edges, however \citep{zoph-arXiv18} require the output of all intermediate nodes to be concatenated as the output of the cell.
Note that the non-linearity applied to the edge weights varies depending on the NAS optimizer used; e.g. for GDAS~\citep{dong2019search} and SNAS~\citep{Xie18} it would be a Gumbel-Softmax~\citep{gumbel} instead. 

\textbf{Choice Blocks.} As in \citet{bender_icml:2018}, each choice block inside the cell can select between the operations in the operations set $\mathcal{O}$ of NAS-Bench-101. In order to find the optimal operation in each choice block via gradient-based one-shot NAS methods, we assign an architectural weight $\beta^o$ to each operation $o \in \mathcal{O}$ inside the choice block. The output of the choice block $j$ is computed by adding element-wise the latent representations coming from the operations outputs: 
\begin{equation} \label{eq:block_output}
\begin{split}
x^j = \sum_{o\in\mathcal{O}}\frac{\exp(\beta^{o})}{\sum_{o^{\prime}\in\mathcal{O}}\exp(\beta^{o^{\prime}})} o(I^j),
\end{split}
\end{equation}
which is basically the so-called \textit{MixedOp} in DARTS.
NASBench cells contain 1x1 projections in front every operation (demonstrated in Figure 1 in \citep{ying19a}). The number of output channels of each projection is chosen such that the output has the same number of channels as the input. This adaptive choice for the number of channels is incompatible with the one-shot model due to the different tensor dimensionality coming from previous choice blocks. We used 1x1 projections with a fixed number of channels instead.


\subsection{Evaluation procedure}
\label{subsec: evaluation_procedure}

By means of these additional weights we do not restrict the possible architectures in the search space to contain only a fixed number of edges per cell, as done for example in \citet{zoph-arXiv18}, \citet{Pham18}, \citet{darts}, etc.
This requirement would have restricted our architectural decisions heavily, leading to only small search spaces. 

\begin{wraptable}[13]{r}{.45\textwidth}
\centering
\vskip -0.19in
\caption{Characteristic information of the search spaces.} % \noteaz{Do we need the last column here?}
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{@{}llccc@{}}
\toprule
\multicolumn{1}{l}{}                                   & \multicolumn{1}{c}{\textbf{}} & \multicolumn{3}{c}{\textbf{Search space}} \\ \midrule
\multicolumn{1}{l}{}                                   &                  & \textbf{1}   & \textbf{2}   & \textbf{3} \\ \cmidrule(l){2-5} 
\multirow{6}{*}{No. parents} & Node 1                        & 1            & 1            & 1          \\
                                                       & Node 2                        & 2            & 1            & 1          \\
                                                       & Node 3                        & 2            & 2            & 1          \\
                                                       & Node 4                        & 2            & 2            & 2          \\
                                                       & Node 5                        & -            & -            & 2          \\
                                                       & Output                        & 2            & 3            & 2          \\ \midrule
\multicolumn{1}{l}{\multirow{3}{*}{No. archs.}} & w/ loose ends                        & 6240         & 29160        & 363648    \\
\multicolumn{1}{l}{}                                   & w/o loose ends                & 3702         & 12510        & 137406    \\  
\multicolumn{1}{l}{}                                   & w/o isomorphism               & 2685         & 7773         & 55854    \\ \bottomrule
\end{tabular}
}
\label{table:search_spaces}
\end{wraptable}

Table \ref{table:search_spaces} shows the characteristics of each search space. We propose three different search spaces by making different decisions on the number of parents each choice block has. The decisions affect the quality and quantity of the architectures contained in each search space. For all search spaces note that the sum of the number of parents of all nodes in the search space is chosen to be 9, to match the NAS-Bench-101 requirement.
Search space 1, 2 and 3 have 6240, 29160 and 363648 architectures with loose ends respectively, making search space 3 the largest investigated search space. To the best of our knowledge search space 3 is currently the largest and only available tabular benchmark for one-shot NAS. For details on each search space see \mbox{Appendix \ref{sec: search_spaces_details}}.

Given the architectural weights of the cell shown in Figure \ref{fig:sec2:overview_graphic} we query the test and validation error of the discrete architecture from NAS-Bench-101 as follows. 
\begin{enumerate}[leftmargin=*]
    \item We determine the operation chosen in each choice block by choosing the operation with the highest architectural weight.
    \item We determine the parents of each choice block and the output by choosing the top-$k$ edges according to Table \ref{table:search_spaces} (e.g. for choice block 4 in search space 3 we would choose the top-2 edges as parents).
    \item From 1. we construct the operation list and from 2. the adjacency matrix of the cell which we use to query NAS-Bench-101 for the test and validation error.
\end{enumerate}

Each node in the graph chooses its parents during evaluation following e.g. DARTS~\citep{darts}. However, because edges model information flow and the output edges are also architectural decisions there is possibility of a node being a loose end. These are nodes whose output does not contribute to the output of the discrete cell, as seen in the upper cell under evaluation of Figure~\ref{fig:sec2:overview_graphic}. As a result, we can count the number of architectures with or without loose ends. Note, that had we chosen the children of each node we could have invalid architectures where a node has an output but no input.




==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/3a_framework.tex <==
\section{A General Framework for One-shot NAS Methods}
\label{sec:framework}

%\notefh{Change flow to make the open-source library of NAS methods, all in the same framework, a contribution.}

%The main advantage of relaxing the architecture space to be continuous by means of the architectural weights $\Lambda =\{ \alpha, \beta, \gamma \}$ comes from the fact that these weights are part of the differentiable computational graph. Therefore, the validation loss $\mathcal{L}_{val}$ is differentiable w.r.t. $\Lambda$, which may be updated using standard gradient descent methods. In general, optimizing both the architectural weighs and the one-shot network parameters is framed as a bi-level optimization problem~\citep{darts}, where:
%\begin{enumerate}
%    \item Updates of network parameters $w$ by $\nabla_w \mathcal{L}_{train}(w, \Lambda)$,
%    \item Updates of architectural parameters $\Lambda$ by $\nabla_{\Lambda} \mathcal{L}_{valid}(w, \Lambda)$,
%\end{enumerate}
%alternate throughout the search. 
Most of the follow-up works of DARTS (Algorithm \ref{alg:darts}), which focus on making the search even more efficient and effective, started from the original DARTS codebase\footnote{\url{https://github.com/quark0/darts}},
and each of them only change very few components compared to DARTS. 

\begin{minipage}{0.24\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{DARTS}\label{alg:darts}
    \footnotesize
    \begin{algorithmic}[1]
        \State \tiny{$I^j = \sum_{i<j} S(\alpha^{i,j}) x^i$}
        \State \tiny{$O^k = \oplus_{j<k} S(\gamma^{j,k}) x^j$}
        \State \tiny{$x^j = \sum_{o\in\mathcal{O}}S(\beta^{o}) o(I^j)$}
        \State \text{m $\gets$ DAG($I^j, O^k, x^j$)}
        \While{not converged}
        \State \text{m.update($\Lambda$, $\nabla_{\Lambda} \mathcal{L}_{valid}$)}
        \State \text{m.update($w$, $\nabla_w \mathcal{L}_{train}$)}
        \EndWhile
        \State \textbf{Return}  \text{$\Lambda$}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{PC-DARTS}\label{alg:pcdarts}
    \footnotesize
    \begin{algorithmic}[1]
        \State \tiny{$I^j = \sum_{i<j} S(\alpha^{i,j}) x^i$}
        \State \tiny{$O^k = \oplus_{j<k} S(\gamma^{j,k}) x^j$}
        \State \tiny{$x^j = \sum_{o\in\mathcal{O}}S(\beta^{o}) o($\hl{$M^o \ast$}$ I^j) $\hl{$+ (1- M^o \ast I^j)$}}
        \State \text{m $\gets$ DAG($I^j, O^k, x^j$)}
        \While{not converged}
        \State \text{m.update($\Lambda$, $\nabla_{\Lambda} \mathcal{L}_{valid}$)}
        \State \text{m.update($w$, $\nabla_w \mathcal{L}_{train}$)}
        \EndWhile
        \State \textbf{Return}  \text{$\Lambda$}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill \sethlcolor{green}
\begin{minipage}{0.32\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{GDAS}\label{alg:gdas}
    \footnotesize
    \begin{algorithmic}[1]
        \State \tiny{$I^j = \sum_{i<j}$\hl{GS}$(\alpha^{i,j}) x^i$}
        \State \tiny{$O^k = \oplus_{j<k}$\hl{GS}$(\gamma^{j,k}) x^j$}
        \State \tiny{$x^j = \sum_{o\in\mathcal{O}}$\hl{GS}$(\beta^{o}) o(I^j)$} 
        \State \text{m $\gets$ DAG($I^j, O^k, x^j$)}
        \While{not converged}
        \State \text{m.update($\Lambda$, $\nabla_{\Lambda} \mathcal{L}_{valid}$)}
        \State \text{\hl{m.update\_single\_path($w$, $\nabla_w \mathcal{L}_{train}$)}}
        \EndWhile
        \State \textbf{Return}  \text{$\Lambda$}
    \end{algorithmic}
\end{algorithm}
\end{minipage}

\sethlcolor{pink}
\begin{minipage}{0.49\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{Random NAS with Weight-sharing}\label{alg:RandomNAS}
    \footnotesize
    \begin{algorithmic}[1]
        \State \tiny{$I^j = \sum_{i<j}$ \hl{$x^i$}}
        \State \tiny{$O^k = \oplus_{j<k}$ \hl{$x^j$}}
        \State \tiny{$x^j = \sum_{o\in\mathcal{O}}$ \hl{$o(I^j)$}}
        \State \text{m $\gets$ DAG($I^j, O^k, x^j$)}
        \While{not converged}
        \State \text{\hl{arch $\gets$ sample\_uniformly\_at\_random(m)}}
        \State \text{\hl{m.update\_weights\_of\_single\_architecture(arch, $w$, $\nabla_w \mathcal{L}_{train}$)}}
        \State 
        \EndWhile
        \For{\hl{i $\in$ 1..1000}}
        \State \text{\hl{arch\_samples $\gets$ sample\_uniformly\_at\_random(m)}}
        \EndFor
        \State \textbf{Return} \hl{arch $\in$ arch\_samples with lowest validation error}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{ENAS}\label{alg:enas}
    \footnotesize
    \begin{algorithmic}[1]
        \State \tiny{$I^j = \sum_{i<j}$ \hl{$x^i$}}
        \State \tiny{$O^k = \oplus_{j<k}$ \hl{$x^j$}}
        \State \tiny{$x^j = \sum_{o\in\mathcal{O}}$ \hl{$o(I^j)$}}
        \State \text{m $\gets$ DAG($I^j, O^k, x^j$)}
        \While{not converged}
        \sethlcolor{cyan}
        \State \text{\hl{arch $\gets$ sample\_using\_controller(m)}}
        \sethlcolor{pink}
        \State \text{\hl{m.update\_weights\_of\_single\_architecture(arch, $w$, $\nabla_w \mathcal{L}_{train}$)}}
        \sethlcolor{cyan}
        \State \hl{Update RNN controller}
        \EndWhile
        \For{\hl{i $\in$ 1..100}}
        \State \text{\hl{arch\_samples $\gets$ sample\_using\_controller(m)}}
        \EndFor
        \sethlcolor{pink}
        \State \textbf{Return} \hl{arch $\in$ arch\_samples with lowest validation error}
    \end{algorithmic}
\end{algorithm}
\end{minipage}

Algorithm \ref{alg:pcdarts} and Algorithm \ref{alg:gdas} highlight these components (relative to DARTS) for PC-DARTS~\citep{xu2019pcdarts} and GDAS~\citep{dong2019search}, respectively. 
For example, when comparing PC-DARTS and DARTS, the only difference in our benchmark is the partial channel connections (line 3 of Algorithm \ref{alg:pcdarts}) in the choice blocks, which consists of a channel sampling mask $M^o$ that drops feature maps coming from $I^j$. 
GDAS, on the other hand, replaces the Softmax (\emph{S)} function in DARTS by a Gumbel-Softmax (\emph{GS}), which applies for every architectural weight in $\Lambda =\{ \alpha, \beta, \gamma \}$ (lines 1-3 in Algorithm \ref{alg:gdas}), and uses this concrete distribution to sample single paths through the cell during search (line 7 in Algorithm \ref{alg:gdas}).
%
Random Search with Weight Sharing (Random WS)~\citep{li2019random} (Algorithm \ref{alg:RandomNAS}) and ENAS~\citep{Pham18} (Algorithm \ref{alg:enas}) do not need the continuous relaxation in order to conduct the architecture search, instead they sample randomly in RandomWS or from the recurrent neural network controller (line 6 in Algorithm \ref{alg:darts}) in ENAS, in order to select the sub-network in the one-shot model to train.

\begin{figure}[b]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99999\textwidth]{imgs/experiments/optimizer_comparison/optimizer_comparison_ss_1_50_test_errors.pdf}
  \caption{Search space 1}
  \label{fig:sec3:ss1_opt}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99999\textwidth]{imgs/experiments/optimizer_comparison/optimizer_comparison_ss_2_50_test_errors.pdf}
  \caption{Search space 2}
  \label{fig:sec3:ss2_opt}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99999\textwidth]{imgs/experiments/optimizer_comparison/optimizer_comparison_ss_3_50_test_errors.pdf}
  \caption{Search space 3}
  \label{fig:sec3:ss3_opt}
\end{subfigure}
\caption{Comparison of different one-shot NAS optimizers on the three different search spaces defined on NASBench. The solid lines show the anytime test regret (mean $\pm$ std), while the dashed blurred lines the one-shot validation error (Best viewed in color).}
\label{fig:sec3:optimizers:comparison}
\end{figure}

These close correspondences between current one-shot NAS variants provide an opportunity to implement all of these variants in the same general code basis.
This allows us to (a) automatically guard against any confounding factors when evaluating the strengths and weaknesses of different approaches, and (b) allows us to mix and match the components of different algorithms. 
%The latter will be particularly interesting when many different one-shot NAS methods have been implemented in the framework.
%
We implemented all variants in a single code basis, which we are committed to grow into a flexible library of primitives for one-shot NAS methods, and for which we will gladly accept any help the community wants to provide.
%that allows users to conduct scientific research in a single framework without having to worry about confounding factors.

One-shot NAS methods in this code basis inherit all the methods and attributes necessary for building the one-shot computational graph from a base parent class. 
This encapsulation and modularity ensures that all differences in their performance come from a few lines of code, and that all other confounding factors cannot affect these results. This will also facilitate the incorporation of other one-shot NAS methods and pinpoint the components that differ in them.

Furthermore, the primitives encoding the search spaces presented in Section \ref{sec:methodology} are defined separately from the NAS optimizers. This encapsulation will 
allow researchers to study each of these components in isolation, experimenting with one of them while being sure that the other one does not change.
%to conduct proper scientific comparisons between NAS methods (where the only difference comes from the contributed search strategy.

%To eliminate confounding factors, which would hinder a fair comparison of the optimizers, we implemented all NAS optimizers to rely on the same code base and only change their contributed search strategy. All optimizers that we chose used the original code base of DARTS in PyTorch \citep{paszke2017automatic}. This means that all gradient based optimizers used the same hyperparameters and were trained on a single NVIDIA RTX2080Ti using the same python environment.

==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/4_experiments.tex <==
\section{NAS-Bench-1Shot1 as a benchmark and analysis framework}
\label{sec:experiments}

We now demonstrate the use of NAS-Bench-1Shot1 as a benchmark for one-shot NAS. We first evaluate the anytime performance of five different one-shot NAS methods: DARTS~\citep{darts}, GDAS~\citep{dong2019search}, PC-DARTS~\citep{xu2019pcdarts}, ENAS \citep{Pham18} and Random Search with Weight Sharing (Random WS) \citep{li2019random}.\footnote{Details on these optimizers can be found in Appendix \ref{sec:app:optimizers}.} Afterwards, we investigate the robustness of these one-shot NAS optimizers towards their search  hyperparameters and show that if these hyperparameters are carefully tuned, the one-shot NAS optimizer can outperform a wide range of other discrete NAS optimizers in our search spaces.

\subsection{Comparison of different One-shot NAS optimizers}
\label{subsec: comparison}

We ran the NAS search for 50 epochs\footnote{This required different amounts of time: DARTS 1st order: 3h, DARTS 2nd order: 4h, GDAS: 1.5h, PC-DARTS: 2h, ENAS: 4h, Random-WS: 11h.} using their respective default hyperparameter settings (see Appendix \ref{sec: hyperparameters}).
If not stated otherwise, all the following results were generated by running each experiment with six random seeds (0 to 5). All plots show the mean and standard deviation of the test regret queried from NAS-Bench-101. Over the three independent trainings contained in NASBench-101 for each architecture on each epoch budget we average. The search was done on a single NVIDIA RTX2080Ti using the same python environment. In Figure \ref{fig:sec3:optimizers:comparison} we report the anytime test regret for each of these methods. Our findings can be summarized as follows:

\begin{itemize}[leftmargin=*]
    \item The test error (queried from NAS-Bench-101) for DARTS, GDAS and PC-DARTS decreases along with the validation error of the one-shot model. However, these two quantities are not necessarily correlated. One such example is the learning curve of PC-DARTS. While the validation error smoothly decreases, the test error of the found solutions slightly goes up in the beginning and then decreases again. This behavior becomes even more substantial when increasing the number of search epochs (see Appendix~\ref{sec: more_search_epochs}). Figure~\ref{fig:sec3:optimizers:comparison_200} shows that when running DARTS for 200 epochs, the test regret diverges. The same result was also previously observed by \citet{zela19} on subspaces of the standard DARTS space.
    \item The ranking of the NAS optimizers differs across search spaces. For instance, while PC-DARTS performs the best in search space 1, this is clearly not the case in the other search spaces. 
    \item GDAS has a better anytime performance than the other optimizers in all 3 benchmarks, however, due to the temperature annealing of the Gumbel Softmax, it manifests some premature convergence (in less than 5 search epochs) to a sub-optimal local minimum.
    \item Random WS and ENAS mainly explore poor architectures across all three search spaces. This behaviour is a result of the small correlation between the architectures evaluated with the one-shot weights and their true performance during architecture evaluation (as queried from NAS-Bench-101 (see Section \ref{sec:corr_analysis})). This correlation directly affects these methods since in the end of search they sample a certain number of architectures (1000 randomly sampled for Random WS and 100 using the learned controller policy for ENAS) and evaluate them using the one-shot model weights in order to select the architecture which is going to be trained from scratch in the final evaluation phase. When running ENAS for 100 epochs in search space 2 (Figure \ref{fig:sec3:optimizers:comparison_100_epochs} in the appendix) we see that the it performs better than Random WS. ENAS also has a stronger correlation between the sampled architectures and the NAS-Bench-101 architectures for search space 2 (see Section \ref{sec:corr_analysis}).
\end{itemize}


\subsection{Correlation analysis} \label{sec:corr_analysis}
Many one-shot NAS methods, such as ENAS~\citep{Pham18}, NAONet~\citep{Luo2018NeuralAO} or Random WS~\citep{li2019random} select the final architecture by means of the one-shot parameters.
In order to assess if this is optimal we computed the correlation between a given architecture's one-shot test error and its respective NAS-Bench-101 test error, for all 4 available budgets in NAS-Bench-101 on every 10th search epoch. This analysis was performed for all architectures without loose ends in each search space. The only exception is ENAS, for which we decided to evaluate the correlation by sampling 100 architectures (as done by the algorithm after the search has finished to select the one to retrain from scratch) from the controller instead of evaluating every architecture in the search space.

As shown in Figure \ref{fig: correlation_s1_s2_s3}, there is almost no correlation between the weight sharing ranking and the true one (Spearman correlation coeff. between -0.25 and 0.3) during search for DARTS, PC-DARTS, GDAS and Random WS. Only ENAS shows some correlation for search space 2 and some anticorrelation for search spaces 1 and 3. These results agree with the ones reported by \citet{sciuto19} (who could only do this evaluationx on a small search space) and explain the poor performance of Random WS and ENAS on our benchmarks, since the architectures sampled during evaluation and ranked according to their one-shot validation error are unlikely to perform well when evaluated independently. To the best of our knowledge this is the first time that an evaluation of this correlation is conducted utilizing such a large number of architectures in the search space, namely 137406 different architectures for search space 3. We added further experiments on the correlation between the lower fidelity proxy model used in architecture search and the final model from architecture evaluation in the Appendix~\ref{sec:correlation_proxy}.
%Our results demonstrate that increasing the budget of the independent architecture training also leads to an increased positive or negative correlation with the one-shot test performance.

\begin{figure}[t]
\centering
\begin{subfigure}{.325\textwidth}
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_1_darts_w_o_cutout.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_1_gdas.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_1_pc_darts.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_1_enas.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_1_randomws.pdf} 
    \caption{Search space 1}
    \label{fig:sec3:ss1:corr}
\end{subfigure}
\centering
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_2_darts_w_o_cutout.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_2_gdas.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_2_pc_darts.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_2_enas.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_2_randomws.pdf}   
    \caption{Search space 2}
    \label{fig:sec3:ss2:corr}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_3_darts_w_o_cutout.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_3_gdas.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_3_pc_darts.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_3_enas.pdf}\\
    \includegraphics[width=0.99\textwidth]{imgs/experiments/correlation/correlation_ss_3_randomws.pdf}   
    \caption{Search space 3}
    \label{fig:sec3:ss3:corr}
\end{subfigure}
\caption{Correlation between the one-shot validation error and the corresponding NAS-Bench-101 test error for each search space. (Best viewed in color).}
\label{fig: correlation_s1_s2_s3}
\end{figure}


\subsection{Robustness of One-Shot NAS optimizers}
\label{subsec:regulatization}

\citet{zela19} observed that the generalization performance of architectures found by DARTS heavily depends on the hyperparameters used during the search phase. More specifically, they investigate regularization hyperparameters that shape the inner objective landscape, such as $L_2$ regularization or CutOut~\citep{cutout} and ScheduledDropPath~\citep{zoph-arXiv18}.

Due to the fast queries from NAS-Bench-101, NAS-Bench-1Shot1 enables researchers to assert if their one-shot NAS optimizers with some specified hyperparameter settings overfit on the validation set during search~\citep{zela19}. In Figure~\ref{fig:sec3:regularization:l2_ss3} we plot the anytime performance of DARTS, GDAS and PC-DARTS on Search Space 3 when ran with different $L_2$ factors in the inner objective (see Appendix~\ref{sec: regularization} for more results on other search spaces and regularizers such as CutOut). Based on these results we observe that:
%As already observed by \citet{zela19}, DARTS tends to become more robust and find better solutions when the inner objective $\mathcal{L}_{train}$ in the bi-level optimization procedure has a relatively strong regularization factor during search. 
%In order to investigate the long term behaviour, for this analysis we chose to run every search for 100 epochs instead of 50 epochs.
%Similarly to \citet{zela19}, we find that enabling Cutout~\citep{cutout} or increasing the $L_2$ factor for the search model weights, has a substantial effect on the quality of the solutions found by the NAS optimizers. See Figure \ref{fig:sec3:regularization:cutout} for the Cutout (CO) results and Figure \ref{fig:sec3:regularization:l2_ss3} (in the appendix) for the results with different $L_2$ regularization. 

%%%%%%%%%%%%%%%% ss3
\begin{figure}[ht]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99\textwidth]{imgs/experiments/regularization/l2_regularization/weight_decay_search_space_3_twin_x_test_errors.pdf}
  \caption{DARTS}
  \label{fig:sec3:ss3_l2}
\end{subfigure}
\begin{subfigure}{.325\textwidth}
  \centering
\includegraphics[width=0.99\textwidth]{imgs/experiments/regularization/l2_regularization/gdas/gdas_weight_decay_search_space_3_twin_x_test_errors.pdf}
  \caption{GDAS}
  \label{fig:sec3:reg:l2_gdas_3}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99\textwidth]{imgs/experiments/regularization/l2_regularization/pc_darts/pc_darts_weight_decay_search_space_3_twin_x_test_errors.pdf}
  \caption{PC-DARTS}
  \label{fig:sec3:reg:l2_pc_darts_3}
\end{subfigure}
\caption{The impact that weight decay has on the test (one-shot validation) performance of architectures found by DARTS, GDAS and PC-DARTS on search space 3 (Best viewed in color).} 
\label{fig:sec3:regularization:l2_ss3}
\end{figure}

\begin{itemize}[leftmargin=*]
    \item Interestingly, while \citet{zela19} only showed overfitting behavior for DARTS, it may also occur for GDAS and PC-DARTS as shown Figure \ref{fig:sec3:reg:l2_gdas_3} and \ref{fig:sec3:reg:l2_pc_darts_3}. This indicates that this might be an intrinsic property of these methods due to the local updates in the architecture space.
    \item A good hyperparameter setting for one NAS optimizer is not necessarily good for others. In Figure~\ref{fig:sec3:regularization:l2_ss3} we can see that for $L_2 = 27\cdot 10^{-4}$ GDAS and PC-DARTS have the best anytime performance, whilst in DARTS we notice an overfitting behavior for the same value.
    \item Interestingly enough, it seems that these NAS optimizers show the same pattern across search spaces for the same $L_2$ values as shown in Figure~\ref{fig:sec3:regularization:l2_ss1} and Figure~\ref{fig:sec3:regularization:l2_ss2} in Appendix~\ref{sec: regularization}.
\end{itemize}


\subsection{Tunability of One-Shot NAS hyperparameters} \label{subsec: bohb_darts}

Next to the hyperparameters used in the evaluation pipeline, one-shot NAS methods have several hyperparameters of their own, such as the regularization hyperparameters studied in Section \ref{subsec:regulatization}, learning rates, and other hyperparameters of the search phase.

\begin{figure}[ht]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99\textwidth]{imgs/bohb/s1-cs2.pdf}
  \caption{Search space 1}
  \label{fig:bohb-s1-cs2}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99\textwidth]{imgs/bohb/s2-cs2.pdf}
  \caption{Search space 2}
  \label{fig:bohb-s2-cs2}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
\includegraphics[width=0.99\textwidth]{imgs/bohb/s3-cs2.pdf}
  \caption{Search space 3}
  \label{fig:bohb-s3-cs2}
\end{subfigure}
\caption{Optimizing the hyperparameters of one-shot optimizers with BOHB on NAS-Bench-1Shot1. Every curve shows the mean$\pm$std of the incumbent trajectories (500 and 3 search repetitions for the black-box and one-shot optimizers, respectively).}
\label{fig:bohb-cs2}
\end{figure}

%\begin{wrapfigure}[16]{r}{0.55\textwidth}
%\vskip -0.25in
%  \centering
%  \includegraphics[width=.55\textwidth]{imgs/bohb/s3-run0-seed1.png}\\
%  \caption{Optimizing the hyperparameters of one-shot optimizers with BOHB on search space 3. (best viewed in color). Results for search space 1 and 2 are shown in Figure \ref{fig:bohb-c1-1st}.}
%  \label{fig:bohb_pcdarts_gdas}
%\end{wrapfigure}

Naively tuning these hyperparameters with the one-shot validation error as the objective would lead to sub-optimal configurations, since, as we saw, this metric is not a good indicator of generalization.
In our proposed benchmarks, we can tune these hyperparameters of the NAS optimizer to minimize the validation error queried from NAS-Bench-101. By doing so, we aim to shed more light onto the influence these hyperparameters have during the one-shot search, and to study the sensitivity of the NAS method towards these hyperparameters.

To this end, we constructed 3 configuration spaces of increasing cardinality, CS1, CS2 and CS3 (see Appendix \ref{sec: bohb_details} for details), which only include hyperparameters controlling the NAS process. We chose BOHB (\cite{Falkner18}, see Appendix \ref{sec: bohb_details} for details) as the hyperparameter optimization method and DARTS (1st order), GDAS, PC-DARTS as our NAS methods to be tuned across all configuration spaces.

Starting from the respective default hyperparameter settings of each one-shot optimizer, we run BOHB with a total budget of 280 function evaluations, where in this case a function evaluation is a query from NAS-Bench-101.
Note that we never use the validation set split used to evaluate the individual architectures in NAS-Bench-101 during the architecture search. This subset with 10k examples is only used to compute the objective function value that BOHB optimizes. Therefore, the one-shot optimizers use 20k examples for training and 20k for the architectural parameter updates.
Figure \ref{fig:bohb-cs2} shows the anytime test regret of the architectures found by the respective NAS method's configurations tried by BOHB on CS2 (see Figure~\ref{fig:bohb-cs1} for results on CS1 and Figure~\ref{fig:bohb-cs3} for results on CS3). The x-axis in these figures shows the \textit{simulated wall-clock time}: $t_{sim}=t_{search}+t_{train}$, where $t_{search}$ is the time spent during search by each configuration and $t_{train}$ is the training time for 108 epochs (queried from NAS-Bench-101) of the architectures selected by the one-shot optimizer. As the figure shows, DARTS, PC-DARTS and GDAS can be tuned to find solutions closer to the global minimum compared to the default hyperparameter settings. 
We note that carrying out this optimization on NAS-Bench-1Shot1 reduced the time for tuning DARTS from a simulated 45 GPU days to 1 day on 16 GPUs.

Figure \ref{fig:bohb-cs2} also provides an evaluation of DARTS, GDAS and PC-DARTS compared to the state-of-art discrete NAS optimizers used by \citet{ying19a} (such as RL, RE, and HPO methods). Since these one-shot NAS methods are much faster than black-box methods, it is possible to tune them \emph{online} using BOHB and the resulting BOHB-$\{$DARTS, GDAS, PC-DARTS$\}$ typically still yields better performance over time. 
From this experiment, we make the following observations:

\begin{itemize}[leftmargin=*]
    \item Across all search spaces the architectures found using the best BOHB configurations outperformed the architectures found by the default DARTS configuration by up to a factor of 10.
    \item As in NAS-Bench-101, Regularized Evolution~\citep{real-arXiv18a} performed the best in all search spaces of NAS-Bench-1Shot1 compared to the other black-box optimizers.
    %, and also outperformed all other discrete NAS optimizers.
    \item The found robust configurations did not only avoid overfitting in the architectural level, but they also typically outperformed the architectures found by state-of-art discrete NAS optimizers used by \citet{ying19a} (such as RL, RE, and HPO methods). %The only exception is on search space 1, where BOHB-DARTS performed on par with RE and SMAC. We attribute this to small search space size and the effectiveness of global optimization methods on such spaces. Whilst, for larger search spaces such as search space 2 and 3 gradient-based methods are faster and more likely to find a good local minimum for the given search budget.
    %\item The best results were obtained from DARTS runs that only used 25 epochs (not the 50 or 100 epochs that were also tried). This was found as a side-effect of using the number of epochs as the budget of the multi-fidelity optimization approach BOHB.
    \item The multi-fidelity in BOHB does not only accelerate the hyperparameter optimization procedure, but in this case also allows to determine the sufficient number of epochs to run the NAS optimizer in order to get an optimal architecture. In fact, the best configuration on each of the incumbents comes usually from the lowest budget, i.e. 25 search epochs.
    %For each of the budgets, BOHB exploits more robust DARTS configurations throughout its optimization procedure. The most robust configuration on each of the search spaces are the ones with a large regularization factor, relative to the default value in \citet{darts} (see Figure \ref{fig:fanova_c1_1st} in the Appendix).
\end{itemize}


==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/5_conclusions.tex <==
\section{Conclusion and Future Directions}
\label{sec: conclusion}

We proposed NAS-Bench-1Shot1, a set of 3 new benchmarks for one-shot neural architecture search which allows to track the trajectory and performance of the found architectures computationally cheaply. Using our analysis framework, we compared state-of-the-art one-shot NAS methods and inspected the robustness of the methods and how they are affected by different hyperparameters. Our framework allows a fair comparison of any one-shot NAS optimizer and discrete NAS optimizers without any confounding factors.
We hope that our proposed framework and benchmarks will facilitate the evaluation of existing and new one-shot NAS methods, improve reproducibility of work in the field, and lead to new insights on the underlying mechanisms of one-shot NAS.



==> 2020 ICLR_ Benchmarking and Dissecting One-shot Neural Architecture Search/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

